Human-Centered Explainable AI (XAI): From Algorithms to User Experiences

In recent years, the field of explainable AI (XAI) has produced a vast collection of algorithms, providing a useful toolbox for researchers and practitioners to build XAI applications. With the rich application opportunities, explainability is believed to have moved beyond a demand by data scientists or researchers to comprehend the models they develop, to an essential requirement for people to trust and adopt AI deployed in numerous domains. However, explainability is an inherently human-centric property and the field is starting to embrace human-centered approaches. Human-computer interaction (HCI) research and user experience (UX) design in this area are becoming increasingly important. In this chapter, we begin with a high-level overview of the technical landscape of XAI algorithms, then selectively survey our own and other recent HCI works that take human-centered approaches to design, evaluate, and provide conceptual and methodological tools for XAI. We ask the question "what are human-centered approaches doing for XAI" and highlight three roles that they play in shaping XAI technologies by helping navigate, assess and expand the XAI toolbox: to drive technical choices by users' explainability needs, to uncover pitfalls of existing XAI methods and inform new methods, and to provide conceptual frameworks for human-compatible XAI.

==> abstract.tex <==
% Although AI holds promise for improving human decision making in critical task such as recidivism prediction and medical diagnosis, models still make occasional errors and are often unpredictable.
% To achieve both human accountability and model precision, human-model collaborations are necessary.
% In this paper, instead of direct collaboration where the human makes a decision given model assistance, we propose conditional delegation, an alternative paradigm for human-model collaboration where the human creates rules about when to trust or distrust the model.
% We use content moderation as a testbed to explore conditional delegation and develop novel interfaces to support interactions that allow humans to maximize model assistance in creating rules for content moderation.
% Using pilot studies and large-scale randomized experiments across two tasks, we demonstrate that model assistance helps humans in creating rules that improves model's precision.
% While model assistance improves efficiency and increase humans' confidence, they may not lead to higher satisfaction with the task.
% Overall, our work points out challenges and future directions towards enhancing human-model collaborations with conditional delegation.


% Despite impressive performance in many benchmark datasets, AI models can still make mistakes, especially for out-of-distribution examples.
% It remains an open question how such imperfect models can effectively work with humans.
% Prior work has focused on exploring AI assistance in helping people make individual high-stake decisions such as recidivism prediction, this paradigm is less appropriate for a large amount of relatively low-stake decisions, e.g., moderating tens of thousands of comments.
% Instead, we propose conditional delegation as an alternative paradigm for human-AI collaboration where the human creates rules about when to trust or distrust the model.
% We use content moderation as a test bed to explore conditional delegation and develop novel interfaces to assist humans in creating rules for conditional delegation, thus identifying trustworthy regions of a model.
% We use two datasets to simulate in-distribution and out-of-distribution scenarios.
% Through randomized experiments, we demonstrate that model assistance helps humans in creating rules that improve the model's precision for both scenarios.
% Furthermore, explanations can improve human efficiency and confidence for the in-distribution case, while improving human performance at the cost of mental efforts in the out-of-distribution case.
% Overall, our work points out challenges and future directions towards enhancing human-model collaborations with conditional delegation.
% \chenhao{I am fine with not having the final sentence.}


Despite impressive performance in many benchmark datasets, AI models can still make mistakes, especially among out-of-distribution examples. 
It remains an open question how such imperfect models can be used effectively in collaboration with humans.
Prior work has focused on AI assistance that helps people make individual high-stakes decisions, which is not scalable for a large amount of relatively low-stakes decisions, e.g., moderating social media comments. 
Instead, we propose conditional delegation as an alternative paradigm for human-AI collaboration where humans create rules to indicate trustworthy regions of a model. Using content moderation as a testbed and leveraging two datasets to simulate \ind and \ood scenarios, we develop novel interfaces to assist humans in creating conditional delegation rules and conduct a randomized experiment. 
Our study demonstrates the promise of conditional delegation in improving model performance and provides insights into design for this novel paradigm, including the effect of AI explanations.

% Furthermore, explanations of model predictions can improve human efficiency and confidence.
% for in-distribution examples, while improving human performance at the cost of mental efforts in out-of-distribution examples.
% \viv{150 words}


==> book chapter (2)/abstract.tex <==
% Although AI holds promise for improving human decision making in critical task such as recidivism prediction and medical diagnosis, models still make occasional errors and are often unpredictable.
% To achieve both human accountability and model precision, human-model collaborations are necessary.
% In this paper, instead of direct collaboration where the human makes a decision given model assistance, we propose conditional delegation, an alternative paradigm for human-model collaboration where the human creates rules about when to trust or distrust the model.
% We use content moderation as a testbed to explore conditional delegation and develop novel interfaces to support interactions that allow humans to maximize model assistance in creating rules for content moderation.
% Using pilot studies and large-scale randomized experiments across two tasks, we demonstrate that model assistance helps humans in creating rules that improves model's precision.
% While model assistance improves efficiency and increase humans' confidence, they may not lead to higher satisfaction with the task.
% Overall, our work points out challenges and future directions towards enhancing human-model collaborations with conditional delegation.


% Despite impressive performance in many benchmark datasets, AI models can still make mistakes, especially for out-of-distribution examples.
% It remains an open question how such imperfect models can effectively work with humans.
% Prior work has focused on exploring AI assistance in helping people make individual high-stake decisions such as recidivism prediction, this paradigm is less appropriate for a large amount of relatively low-stake decisions, e.g., moderating tens of thousands of comments.
% Instead, we propose conditional delegation as an alternative paradigm for human-AI collaboration where the human creates rules about when to trust or distrust the model.
% We use content moderation as a test bed to explore conditional delegation and develop novel interfaces to assist humans in creating rules for conditional delegation, thus identifying trustworthy regions of a model.
% We use two datasets to simulate in-distribution and out-of-distribution scenarios.
% Through randomized experiments, we demonstrate that model assistance helps humans in creating rules that improve the model's precision for both scenarios.
% Furthermore, explanations can improve human efficiency and confidence for the in-distribution case, while improving human performance at the cost of mental efforts in the out-of-distribution case.
% Overall, our work points out challenges and future directions towards enhancing human-model collaborations with conditional delegation.
% \chenhao{I am fine with not having the final sentence.}


Despite impressive performance in many benchmark datasets, AI models can still make mistakes, especially among out-of-distribution examples. 
It remains an open question how such imperfect models can be used effectively in collaboration with humans.
Prior work has focused on AI assistance that helps people make individual high-stakes decisions, which is not scalable for a large amount of relatively low-stakes decisions, e.g., moderating social media comments. 
Instead, we propose conditional delegation as an alternative paradigm for human-AI collaboration where humans create rules to indicate trustworthy regions of a model. Using content moderation as a testbed and leveraging two datasets to simulate \ind and \ood scenarios, we develop novel interfaces to assist humans in creating conditional delegation rules and conduct a randomized experiment. 
Our study demonstrates the promise of conditional delegation in improving model performance and provides insights into design for this novel paradigm, including the effect of AI explanations.

% Furthermore, explanations of model predictions can improve human efficiency and confidence.
% for in-distribution examples, while improving human performance at the cost of mental efforts in out-of-distribution examples.
% \viv{150 words}

